Geodesic Convolutional Shape Optimization

Aerodynamic shape optimization has many industrial applications. Existing methods, however, are so computationally demanding that typical engineering practices are to either simply try a limited number of hand-designed shapes or restrict oneself to shapes that can be parameterized using only few degrees of freedom. In this work, we introduce a new way to optimize complex shapes fast and accurately. To this end, we train Geodesic Convolutional Neural Networks to emulate a fluidynamics simulator. The key to making this approach practical is remeshing the original shape using a polycube map, which makes it possible to perform the computations on GPUs instead of CPUs. The neural net is then used to formulate an objective function that is differentiable with respect to the shape parameters, which can then be optimized using a gradient-based technique. This outperforms state- of-the-art methods by 5 to 20% for standard problems and, even more importantly, our approach applies to cases that previous methods cannot handle.

==> figures/airfoil2D.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[thbp]
	\captionsetup[subfigure]{labelformat=empty}
	\centering
	\begin{minipage}{.23\textwidth}
	{\includegraphics[width=35mm, trim={60 0 60 0},clip]{figures/fig_regressor2D/icml_10.pdf}}
	\end{minipage}
	\begin{minipage}{.23\textwidth}
	{\includegraphics[width=35mm, trim={60 0 60 0},clip]{figures/fig_regressor2D/icml_16.pdf}}
	\end{minipage}
	\begin{minipage}{.23\textwidth}
	{\includegraphics[width=35mm, trim={60 0 59 0},clip]{figures/fig_regressor2D/icml_130.pdf}}
	\end{minipage}
	\begin{minipage}{.23\textwidth}
	{\includegraphics[width=35mm, trim={60 0 59 0},clip]{figures/fig_regressor2D/icml_144.pdf}}
	\end{minipage}
	\caption{We visualize the performance of the proposed  geometric predictor on the validation set. In a single visualization we illustrate the CNN \textcolor{blue}{input shape}, where dots show the discretization resolution, the pressure distribution respectively along \textcolor{red}{top} and \textcolor{green}{bottom} of the airfoil and \textcolor{orange}{drag} via an intensity histogram. Ground truth values are reported with dashed lines.  }
	\label{fig:airfoil2D}
\end{figure}

\begin{figure}[thbp]
	\centering
	{\includegraphics[width=80mm, trim={0 0 0 0},clip]{figures/fig_gaussianprocesses/fig.png}}	
	\caption{We compare the performance of the \textcolor{cyan}{GP predictor} to a \textcolor{green}{KNN predictor} and the proposed \textcolor{red}{ geometric CNN predictor} on the NACA data-set. We also report the performance of the proposed CNN trained on the non-parameterized space on the NACA test set. \ER{Producing confidence interval also for CNN.}   }
	\label{fig:comparison2D}
\end{figure}
